OUTformation: Distributed Data-Gathering with Feedback under Unknown Environment and Communication Delay Constraints

Towards the informed design of large-scale distributed data-gathering architectures under real-world assumptions such as nonzero communication delays and unknown environment dynamics, this paper considers the effects of allowing feedback communication from the central processor to external sensors. Using simple but representative state-estimation examples, we investigate fundamental tradeoffs between the mean-squared error (MSE) of the central processor's estimate of the environment state, and the total power expenditure per sensor under more conventional architectures without feedback (INformation) versus those with broadcast feedback (OUTformation). The primary advantage of enabling feedback is that each sensor's understanding of the central processor's estimate improves, which enables each sensor to determine when and what parts of its current observations to transmit. We use theory to demonstrate conditions in which OUTformation maintains the same MSE as INformation with less power expended on average, and conditions in which OUTformation obtains less MSE than INformation at additional power cost. These performance tradeoffs are also considered under settings where environments undergo less variation, and sensors implement random backoff times to prevent transmission collisions. Our results are supported via numerical studies, which show that the properties derived in theory still hold even when some of the simplifying assumptions are removed.

==> sections/prose/related_work.tex <==
\begin{itemize}
    % \item for optimizing backoff time have been discussed in literature (e.g.~\cite{nutt82}) but for the purposes of this paper, 
    % %
    % change-detection on sensors when they have enough power (e.g.~\cite{fearnhead19})
    % However, both are methods which can be used to improve both INformation and OUTformation...
    
    % \item 

    \item Also data fusion is the focus of~\cite{castanedo13}; doesn't consider feedback.
    There have been attempts to reduce latency and computational cost via \textit{hierarchical clustering} of the sensors~\cite{ye02,bandyopadhyay03,younis04}, which require further communication links to be enabled among sensors.
    Even for multiple fusion nodes, feedback is only considered within subgroups of processor nodes, never from processor to sensor~\cite{liggins97}.
    We argue that hierarchical clustering approaches my find some benefits with the additional broadcasting capability included.
    
    \item In literature, there are also a number of \textit{decentralized control} approaches, for which there is no central processor, and the sensors exclusively communicate with each other to exchange information and make decisions for the network. While the framework we propose can be extended to the decentralized controller structure, we focus exclusively on the distributed structure in this work.
    Since making informed decisions requires the central processor to have a good estimate of the environment state, throughout this work we focus on the problem of estimation rather than control.
    Hence, throughout the paper, it is the job of the central processor to fuse the sensors' individual measurements in a smart way to obtain an estimate $\hat{\xvect}(t)$ of the environment's true state $\xvect(t)$.
\end{itemize}


